Minimizing Embedding Distortion for Robust Out-of-Distribution Performance

Foundational models, trained on vast and diverse datasets, have demonstrated remarkable capabilities in generalizing across different domains and distributions for various zero-shot tasks. Our work addresses the challenge of retaining these powerful generalization capabilities when adapting foundational models to specific downstream tasks through fine-tuning. To this end, we introduce a novel approach we call "similarity loss", which can be incorporated into the fine-tuning process of any task. By minimizing the distortion of fine-tuned embeddings from the pre-trained embeddings, our method strikes a balance between task-specific adaptation and preserving broad generalization abilities. We evaluate our approach on two diverse tasks: image classification on satellite imagery and face recognition, focusing on open-class and domain shift scenarios to assess out-of-distribution (OOD) performance. We demonstrate that this approach significantly improves OOD performance while maintaining strong in-distribution (ID) performance.

==> sec/3_background.tex <==
\section{Background}

ORAN: this section should be shortened

\subsection{Contrastive Loss}
Contrastive learning is a representation learning approach, often used in self-supervised learning frameworks such as (ADD REFERENCES) that learns effective representations by contrasting positive pairs against negative pair examples. The core idea is to pull together the representations of an anchor sample and a positive sample of the same class, while pushing apart the representations of the anchor sample and negative samples from different classes. This is typically achieved by optimizing a cross entropy loss function:

\begin{equation}\label{eq:contrastive_loss}
L_{con}(u_i, v_i) = -\log \frac{\exp \left(\operatorname{sim}\left(u_{i}, v_{i}\right) / \tau\right)}{\sum_{j=1}^{N} \exp \left(\operatorname{sim}\left(u_{i}, v_{j}\right) / \tau\right)},
\end{equation}

where $z_i$ is the representation of the anchor sample, $z_j$ is the representation of a positive sample, $\{z_k\}_{k=1}^N$ are representations for $N$ negative examples, $\tau$ is a temperature parameter that controls the smoothness of the distributions, and $\text{sim}(u, v)=u^{\top}v/|u||v|$ is the cosine similarity. Optimizing this loss causes the representations of positive pairs to be pulled together and negative pairs to be pushed apart in the embedding space.
Through the optimization of this loss, the framework encourages the learning of embeddings that are closely aligned for positive pairs and distinctly separated for negative pairs, thereby facilitating the acquisition of robust and generalizable embedding space applicable across diverse tasks.

\subsection{Triplet Loss}
Triplet training is a method used to learn useful representations by comparing relative similarities between data points. It involves taking a triplet of examples --- an anchor $(a)$, a positive instance $(p)$, and a negative instance $(n)$ --- where the anchor is more similar to the positive than to the negative instance. The triplet loss function is designed to ensure that the distance between the anchor and the positive $(D(a, p))$ is smaller than the distance between the anchor and the negative $(D(a, n))$, by at least a margin $(m)$. The triplet loss $(L)$ is formally given by:

\begin{equation}
L(a, p, n) = \max \left( D(a, p) - D(a, n) + m, 0 \right)
\end{equation}

where $D(\cdot)$ is a distance metric, typically the Euclidean distance or cosine distance, and $m > 0$ is a margin that enforces a buffer between positive and negative pairs.

\subsection{Tuning CLIP For Image Classification}
Contrastive Learning in the Pretrained CLIP Model leverages a symmetric contrastive loss function designed to minimize the distance between matched image-text embedding pairs while maximizing the distance between unmatched pairs within a batch. For a given batch of $N$ image-text pairs $(I_i, T_i)_{i=1}^N$, where $I_i$ and $T_i$ denote the $i^{th}$ image and its corresponding text, the symmetric contrastive loss is defined as:

\begin{equation}
\mathcal{L} = \frac{1}{2N} \sum_{i=1}^N \left[ \ell(I_i, T_i) + \ell(T_i, I_i) \right],
\end{equation}
where $\ell(I, T)$ is the loss for a matching image-text pair and is computed by:
\begin{equation}
\ell(I, T) = -\log \frac{\exp(f(I) \cdot g(T) / \tau)}{\sum_{j=1}^N \exp(f(I) \cdot g(T_j) / \tau)}.
\end{equation}

In this formulation, $f(\cdot)$ and $g(\cdot)$ stand for the image and text encoders, respectively, mapping inputs to a common embedding space. The parameter $\tau$ represents the temperature and acts as a scaling factor that modulates the sharpness of the distribution over similarities.

ORAN: need to be more specific about contrastive for classification.
In addition need to elaborate on other methods to learn image classificaation with clip (zero shot, linear layer on top)

\subsection{Face Recognition}

One of the most common use cases in representation learning is for the task of face recognition. Face recognition involves verifying a person's identity by analyzing and comparing two facial images to understand if the images are of the same identity or not. This is usually done by computing an embedding to each facial image, followed by a similarity score calculation between the embeddings. The final decision whether the two images depict the same identity or not is decided by a threshold which is set according to specific application needs.

In order for the embedding space to capture meaningful features that will be able to distinguish between different identities, the key component of this task is to learn a discriminative respresentation.
